Twisted $L^2$-torsion on the character variety

We define a twisted $L^2$-torsion on the character variety of 3-manifold $M$ and study some of its properties. In the case where $M$ is hyperbolic of finite volume, we prove that the $L^2$-torsion is a real analytic function on a neighborhood of any lift of the holonomy representation.

==> FKdet.tex <==
% !TEX root = twistedL2.tex
In this section we conclude the proof of Theorem \ref{theo:Analyticity}, whose statement we recall here:

\begin{theorem}
  The twisted $L^2$-torsion function 
  \[
  \todeux \colon X(M) \to \mR
  \]
  is real-analytic on an analytic neighborhood $U$ of any lift $[\rho_0]$ of the holonomy representation of $M$ in the character variety $X(M)$.
\end{theorem}

In Subsection~\ref{subsec:Comb} and \ref{subsec:L2torsion} we give some more detail about the chain complexes and combinatorial Laplacians that are used to define the $L^2$-torsion in \eqref{defn_todeux}, and give a definition in terms of relative cohomology together with the spectral gap property (Lemma \ref{gap}) that allows us to apply Lemma \ref{analytic_det} to deduce Theorem \ref{theo:Analyticity}. We give the proof of Lemma \ref{gap} in Subsection \ref{subsec:Technical}, using comparison with the analytic $L^2$-invariants and the spectral gap property of the holonomy representation established in \cite[Lemma 4.1]{BV}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Combinatorial Laplacians}
\label{subsec:Comb}
We fix a triangulation of $M$ and denote by $e_j^p, 1 \le j \le n_p$ its $p$-simplices. Let $C_*(\wdt M)$ be the $\CC\pi$-complex of $\mathbb C$-valued chains of the triangulation of $\wdt M$ lifted from that of $M$. We denote by $\partial_p$ the boundary maps of $C_*(\wdt M)$. For each $p, j$ we choose an arbitrary lift $\tilde e_j^p$ of $e_j^p$ to $\wdt M$; these lifts form a basis of $C_*(\wdt M)$ so that we get an isomorphism $C_*(\wdt M) \to (\CC\pi)^{n_p}$. 

Let $\rho$ be a representation of $\pi$ to $\SL_2(\CC)$ and $C_*(\wdt M, \rho)$ the $\CC\pi$-complex $C_*(\wdt M) \otimes_\CC \CC^2$, where the action on $\CC^2$ is trivial---only the boundary maps $\partial_p(\rho)$ will depend on $\rho$. It is immediate to see that this definition of $C_*(\wdt M, \rho)$ gives a complex that is isomorphic to the one used in Section \ref{sec:L2} (see for example \cite[Lemma 1.1]{Lueck_twisted}). To compute the boundary maps we fix an arbitrary basis $(v_1, v_2)$ of $\CC^2$, so that we get a basis $(\tilde e_j^p \otimes v_k)$ of $C_*(\wdt M, \rho)$ as a free $\mC\pi$-module. Then if we write $\partial_p\tilde e_i^p = \sum_{j, \gamma} a_{j, \gamma} \gamma \cdot \tilde e_j^{p-1}$ we have the formula:
\begin{align*}
  \partial_p(\rho)(e_i^p \otimes v_k) &= \sum_{j, \gamma}  a_{j, \gamma} \gamma \cdot (\tilde e_j^{p-1} \otimes \rho(\gamma)v_k) \\
  &= \sum_{j=1}^{n_{p-1}} \sum_{l=1}^2 \left(\sum_{\gamma \in \Gamma} a_{j, \gamma} \cdot \rho(\gamma)_{l, k} \cdot \gamma \right) \cdot (\tilde e_j^{p-1} \otimes v_l)
\end{align*}
where $\rho(\gamma)_{l, k}$ are the coefficients of $\rho(\gamma)$ in the basis $v_1, v_2$. We identify $\partial_p(\rho)$ with its matrix in the bases $(e_i^p \otimes v_k)$, and as the matrix coefficients $\rho \mapsto \rho(\gamma)_{l, k}$ are regular maps on the representation variety $R(M)$ we can subsume the above discussion in the following lemma. 

\begin{lemma} \label{variation_diff}
 There exists a finite subset $S \subset \pi$ and a family of functions $a_s^p : R(M) \to~M(2n_p, 2n_{p-1}, \CC)$ for $s \in S$ and $p=0, 1, 2$, which are regular on a Zariski-neighborhood of the holonomy $\rho_0$ in $R(M)$, such that $\partial_p(\rho) = \sum_{s \in S} a_s^p \cdot s$. 
\end{lemma}

Hence putting $\partial_p(\rho) = \sum_{s \in S} a_s^p(\rho) \cdot s$ we have a complex $C_p(\wdt M, \rho)$ with terms $\CC\pi^{2n_p}$ and boundary maps $\partial_p(\rho)$. The matrix $\partial_p(\rho)$ has finite support and its coefficients are real-analytic on a neighbourhood of $\rho_0$  by Lemma \ref{variation_diff}. Now let $\delta_p(\rho) \in M(n_p, n_{p+1}, \CC)$ be the conjugate transpose matrix of $\partial_p(\rho)$, so we finally define the Laplacian $\Delta_p(\rho) = \delta_p(\rho) \partial_p(\rho) + \partial_{p-1}(\rho) \delta_{p-1}(\rho) \in M(n_p, \CC\pi)$. These functions also have finite support (contained in $S \cup S^{-1}$) and their coefficients are real-analytic. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{$L^2$-torsion} \label{subsec:L2torsion}

\subsubsection{$L^2$-(co)chain complexes} We recall the definition of the $L^2$-chain complexes we work with; we will consider an irreducible character $[\rho] \in X(M)$ and a lift $\rho$ of $[\rho]$ (see Lemma \ref{section}). We put an inner product on the spaces $C_p(\wdt M, \rho)$ by taking the elements $e \otimes v_i$ where $e$ is a simplex and $i=1, 2$, to be an orthonormal basis. This inner product is invariant under the action $\gamma\cdot(e\otimes v) = (\gamma\cdot e) \otimes v$. The Hilbert space completion will be denoted by $C_p^{(2)}(\wdt M, \rho)$; the $\CC\pi$-module structure on $C_p(\wdt M, \rho)$ extends to a $\neu\pi$-Hilbert module structure on $C_p^{(2)}(\wdt M, \rho)$. The Laplacian $\Delta_p(\rho)$ extends to a bounded positive self-adjoint operator on $C_p^{(2)}(\wdt M, \rho)$ which we denote by the same symbol. We use similar definitions and notations for co-chain complexes $C^*_{(2)}(\wdt M, \rho)$. 

Let $i$ be the inclusion $\partial\wdt M \subset\wdt M$, then we have a relative $L^2$ cochain complex $C_{(2)}^*(\wdt M, \partial\wdt M, \rho)$ which fits into the exact sequence
\[
0 \to C_{(2)}^*(\wdt M, \partial\wdt M, \rho) \to C_{(2)}^*(\wdt M, \rho) \xrightarrow{i^*} C^*_{(2)}(\partial\wdt M, \rho\vert_{\partial M}) \to 0. 
\]
We denote by $\Delta_\rel^p$ the combinatorial Laplacians of the complex $C_{(2)}^*(\wdt M, \partial\wdt M, \rho)$. The crucial point for us is then the following, which we prove in the next subsection.  

\begin{lemma} \label{gap}
  There exists $\lambda_0 > 0$ and a neighborhood $U$ of the holonomy such that for all $[\rho] \in U$, for all $p=0, \ldots 3$, we have $\sigma(\Delta_\rel^p(\rho)) \subset \interval f{\lambda_0}{+\infty}o$. 
\end{lemma}

%definition using relative chains/absolute cochains% We could also consider the $L^2$-cochain complex $C^*(\wdt M, \rho)$. An adaptation of the arguments in \cite{Lott_Lueck} shows that it is of determinant class for $\rho$ in $U$ (it seems however that this complex does not have all its Novikov--Shubin invariants equal to $\infty^+$). We can then use the exact sequence associated to the pair $(\wdt M, \partial\wdt M)$, and Poincaré duality (\cite[Theorem 6.7(7)]{Lueck_twisted}) to prove that the $L^2$-torsion thus defined is equal to $\todeux$. 

%%%%%%%%%%%%%%%%%%%%

\subsubsection{Poincar\'e duality} 
We follow the references \cite{Lueck} (see the proofs of Theorems 1.36(3) and 3.93(3)) and \cite[Theorem 6.7(7)]{Lueck_twisted}. There is a homotopy equivalence $P_*\colon C_*(\wdt M) \to~C^{3-*}(\wdt M, \partial\wdt M)$ (the untwisted chain and relative cochain complexes); a construction is given in the proof of Theorem 2.1 in \cite{Wall_surgery_book}. We can extend it by the identity to a homotopy equivalence between the twisted complexes. The Whitehead torsion of $P_*$ vanishes by \cite[Theorem 2.1]{Wall_surgery_book} and it follows that the complexes $C_*(\wdt M, \rho)$ and $C^{n-*}(\wdt M, \partial\wdt M, \rho)$ are homotopy equivalent. By \cite[Theorem 2.19]{Lueck} it follows that they have the same Novikov--Shubin invariants. In particular $\Delta_p(\rho_0)$ has a spectral gap. 

%%%%%%%%%%%%%%%%%%%%

\subsubsection{Proof of Theorem \ref{theo:Analyticity}} The $L^2$-relative cochain complex $C^*(\wdt M, \partial\wdt M, \rho)$ is of determinant class for $\rho$ in the neighbourhood $U$ given by Lemma \ref{gap}. By Poincaré duality (see preceding paragraph) we get that $C_*^{(2)}(\wdt M, \rho)$ is of determinant class and that for $\rho \in U$, $\inf\sigma(\Delta_p(\rho)) > 0$. 

Together with Lemma \ref{variation_diff} this ensures that the hypothese of Lemma \ref{analytic_det} are satisfied by $[\rho] \mapsto \Delta_p(\rho)$ (where $\rho$ belongs to the section of the map $R(M) \to X(M)$ given by Lemma \ref{section}; note also that the spaces on which $\Delta_p(\rho)$ are defined do not depend on $\rho$). It follows from the latter that the functions $[\rho] \mapsto \det_{\neu\pi}\Delta_p(\rho)$ are real-analytic in $U$ and so is the $L^2$-torsion by \eqref{defn_todeux}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of lemma \ref{gap}} \label{subsec:Technical}

\subsubsection{Preliminaries on analytic $L^2$-invariants}
In this subsection we define the twisted analytic Laplacian operators and derive some of their properties.

Let $M$ be a hyperbolic 3-manifold of finite volume, and $\rho \colon \pi_1(M) \to \SL_2(\mC)$ a representation. We consider the trivial rank 2 bundle 
$\HH^3 \times \mC^2$
with the $\pi_1(M)$-action
%Equivalently, $\rho$ defines a flat vector bundle $E_\rho \longrightarrow M$ on $M$ as follows:
%$$E_\rho = \HH^3 \times_\rho \mC^2 = \HH^3 \times \mC^3 / \sim$$
%where $\HH^3 \times \mC^2$ is the trivial bundle of rank 2 on $\HH^3$ and 
$$\gamma \cdot (\widetilde x, v) = (\gamma \cdot \widetilde w, \rho(\gamma) \, v)$$
for any $\gamma \in \pi_1(M), \widetilde x \in \HH^3, v \in \CC^2$.

%We consider the space of $\rho$-twisted differential forms on $M$. They are defined as $\CC^2$-valued differential forms on $\HH^3$ that satisfy equivariance property:
%$$\Omega^*(M, E_\rho) = \lbrace \omega \in \Omega^*(\HH^3, \CC^2) \mid \gamma^*\omega = \rho(\gamma) \,\omega \rbrace$$
We consider the complex $\Omega(\HH^3, \CC^2)$ of $\CC^2$ valued forms on $\HH^3$ with
the natural differential $d_p \colon \Omega^p(\HH^3, \CC^2) \to \Omega^{p+1}(\HH^3, \CC^2)$ 
%preserves equivariance, hence it turns $\Omega^*(M, E_\rho)$ into a complex: the $E_\rho$-valued de Rham complex on $M$.

For any fixed $\rho$, we pick a $\pi_1(M)$-invariant hermitian metric on~$\HH^3 \times \CC^2$. 
%It descends to a hermitan metric on $E_\rho$, and  
It provides a Hodge star operator 
$$\ast_p \colon \Omega^p(\HH^3, \CC^2)) \to \Omega^{3-p}(\HH^3, \CC^2))$$
%by restriction of the Hodge-star operator on the trivial bundle $\HH^3 \times \CC^2$ to equivariant $p$-forms.

We denote by  $\Omega^p_c(\HH^3, \CC^2))$ the space of compactly supported forms in $\Omega^p(\HH^3, \CC^2))$
and we define a hermitian product on compactly supported $p$-forms:
$$
(\phi,\psi)= \int_M \phi\wedge*_p\psi   \qquad \forall\phi,\psi\in \Omega^p_c(\HH^3, \CC^2)),
$$
where $\wedge$ denotes the exterior product on forms in $\Omega^*(\HH^3)$ combined with the hermitian product on $E_\rho$.

Now we define a co-differential $d_{p-1}^* \colon \Omega^{p}(\HH^3, \CC^2)) \to \Omega^{p-1}(\HH^3, \CC^2))$ by the usual formula
$$d_{p-1}^* = (-1)^p (\ast_{p-1})^{-1} \,  d_{3-p} \,  \ast_{p}$$
or equivalently, we define $d_p^*$ being the formal adjoint of $d_p$:
$$(d_p \omega, \eta) = (\omega, d_p^* \eta)$$ 
for any $\omega \in \Omega_c^p(\HH^3, \CC^2)),  \eta \in \Omega_c^{p+1}(\HH^3, \CC^2))$.

The Laplacian is then defined on smooth forms by
\[
\Delta_p \colon \Omega^p(\HH^3, \CC^2)) \to \Omega^p(\HH^3, \CC^2)), \quad \Delta_p = d_p^* d_p + d_{p-1}d_{p-1}^*
\]
It extends uniquely as an essentially self-adjoint operator to $L^2\Omega^*(\HH^3, \CC^2))$. 

%In the sequel we will use or emulate various results about $L^2$-invariants from \cite{Lueck} and \cite{Lott_Lueck}. In our context we deal with the cellular and de Rham complexes with coefficients in a representation $\rho \in R(M)$ but in those references the results are stated for trivial coefficients. However most proofs go through without modifications in our setting (see also \cite{Lueck_twisted}). At some points care is required, in particular we may use Poincaré duality because the representations $\rho$ we consider are self-dual (the determinant gives a $\rho(\Gamma)$-invariant, non-degenerate bilinear form on $\CC^2$).

%The most delicate point is the comparison between analytic and cellular $L^2$-invariants. We will accept that the arguments in \cite[Section 5]{Lott_Lueck} and \cite[Chapter 2]{Lueck} go through for twisted coefficients, once an arbitrary Hermitian metric on the fibers of

%We need to define analytic $L^2$-invariants of the flat vector bundle associated to $\rho$. The space of the bundle over $\HH^3$ (or a subset) is $\HH^3 \times \CC^2$, with diagonal $\pi$-action $\gamma \cdot (x, v) = (\gamma x, \rho(\gamma)v)$. This gives a canonical connection and the associated covariant differential does not depend on $\rho$ (see \cite[Chapter 1.1]{Berline_Getzler_Vergne}), in fact it is defined by $d(\omega\otimes v) = d\omega\otimes v$. Now we choose a smooth $\Gamma$-invariant Hermitian metric on the fibers. %, and we do so so that it depends smoothly on $\rho$.
%In fact we will use this construction only for $\rho=\rho_0$ and in this case there is a canonical choice of metric. 

We use a uniform notation for various spaces of differential forms: if $X$ is a manifold, a prefix $R$ before $\Omega^p(X, \rho)$ indicates that we consider $p$-forms with coefficients in the flat bundle associated to $\rho$ and regularity $R$ (for example $L^2\Omega^p$, $H^l\Omega^p$ for square-integrable and Sobolev spaces). These Hilbert spaces and their $\neu\pi$-module structure depend on $\rho$. 

%There is an associated Hodge Laplacian $\Delta^p(\rho)$ which is an unbounded, essentially selfadjoint operator on $L^2\Omega^p(\HH^3, \rho)$ (which also depend on $\rho$).

The following result essentially follows from \cite[Lemma 4.1]{BV}; we give a short justification as this reference nominally covers only compact locally symmetric spaces\footnote{The statement of \cite[Lemma 4.1]{BV} is given only for the discrete spectrum but the argument also applies to continuous spectrum as the representations in the packets contributing to the spectrum on $p$-forms also satisfy the condition $\mathrm{Hom}_K(\wedge^p\mathfrak p^* \otimes \CC^2, \cdot) \not= 0$ which is the only point used to give a lower bound on the Casimir eigenvalue. Rigorously justifying this would take too much time so we give a suboptimal bootstrap argument below.}. 

\begin{lemma} \label{gap_complete}
  There exists $\delta > 0$ such that for the holonomy $\rho_0$ and $0 \le p \le 3$ we have $\sigma(\Delta^p(\rho_0)) \subset \interval f\delta{+\infty}o$. 
\end{lemma}

\begin{proof}
  Strictly speaking \cite[Lemma 4.1]{BV} (together with 8.2 which checks the hypothesis for the adjoint representation) applies only to the spectrum of compact hyperbolic 3--manifolds. However, by a standard argument using the trace formula (see for example \cite{deGeorge_Wallach}) the normalised spectral measures of a sequence of compact manifolds $M_n$ with $\mathrm{inj}(M_n) \to +\infty$ converge weakly to the spectral measure for $\HH^3$. The spectral gap persists in the weak limit and the existence of such a sequence $M_n$ (which follows from the residual finiteness of the fundamental group of  hyperbolic 3--manifold) guarantees the spectral gap for $\HH^3$. 
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Comparison of analytic and combinatorial invariants for the holonomy} \label{preceding}

The main step in the proof of Lemma \ref{gap} is now to prove the spectral gap for $\rho = \rho_0$. We compare the spectrum of Laplace operators on $C_{(2)}^*(\wdt M, \partial\wdt M, \rho)$ and the Sobolev complexes $H^{l-*}\Omega^*(\HH^3, \rho)$ using Whitney maps. Our arguments are essentially those leading to \cite[Lemma 2.71]{Lueck}. 

First we recall the definition of Whitney maps. We need to use a different model for the cochain complex than the one we used previously: $C^*(\wdt M, \rho) = C^*(\wdt M) \otimes \CC^2$ but with action $\gamma\cdot(f\otimes v) = (\gamma f) \otimes (\rho(\gamma)v)$ and differentials $d(f\otimes v) = (df) \otimes v$; if we fix a $\CC\pi$-basis of $C_p(\wdt M)$ the map $\gamma f \otimes v \mapsto \gamma f \otimes \rho(\gamma)v$ gives an isomorphism of $\CC\pi$-complexes from our former model to this one. We choose a smooth partition of unity $e_c$ on $M$, indexed by vertices $c$ of the triangulation and we lift it to $\wdt M$. The important property that we require is that $e_c$ has its support contained in the open simplices adjacent to $c$. Then, if $f_\sigma$ is the cochain with value 1 on $\sigma$ and $0$ on other simplices we define
\[
W^p(f_\sigma \otimes v) = p! \sum_{c \in \sigma} \omega_{\sigma, c} \otimes v
\]
where $\omega_{\sigma, c}$ is defined by the usual formula: if $c_0, \ldots, c_p$ are the vertices of $\sigma$ ordered according to orientation, $\omega_{\sigma, c_i} = (-1)^ie_{c_i} \cdot \bigwedge_{j \not= i} de_{c_j} $. The form $W^pf_\sigma\otimes v$ is supported in the open star of $\sigma$; in particular it is compactly supported in $\wdt M \setminus \partial\wdt M$ if $\sigma$ is not contained in $\wdt \partial M$. 
  
Thus restricting $W$ defines a map $C^*(\wdt M, \partial\wdt M) \to C_c^\infty\Omega^*(\HH^3)$, and a direct computation (see \cite[p. 140]{Whitney}) shows that it is a chain map---note that in the model we use here, on both sides the differentials satisfy $d(f\otimes v) = df\otimes v$, $d(\omega\otimes v) = d\omega\otimes v$ we can use this computation as it is for our twisted case. This map extends to a bounded chain map $C_{(2)}^*(\wdt M, \partial\wdt M) \to H^{l-*}\Omega^*(\HH^3)$. To prove our claim about the spectral gap of $C_{(2)}^*(\wdt M, \partial\wdt M, \rho)$ it suffices to prove the following inequalities: there exists $C, c > 0$ such that for all $p$ and $f \in C_{(2)}^p(\wdt M, \partial\wdt M, \rho)$ we have 
\begin{equation} \label{lipschitz}
c\|f\|_{L^2} \le \|W^pf\|_{H^{l-p}} \le C\|f\|_{L^2}.
\end{equation}
Indeed, if this holds then for any $f$ the Rayleigh quotient of $W^pf$ satisfies
\[
\frac{ \|d(W^pf)\|_{H^{l-p-1}}^2 } {\|W^pf\|_{H^{l-p}}} = \frac{ \|W^p(df)\|_{H^{l-p-1}}^2 } {\|W^pf\|_{H^{l-p}}} \le (c^{-1}C) \frac{\|df\|_{L^2}} {\|f\|_{L^2}}
\]
and by Lemma \ref{gap_complete} it follows that we must have $\frac{\|df\|_{L^2}} {\|f\|_{L^2}} \ge \frac c C \delta$. 

The content of \eqref{lipschitz} is the minoration $c\|f\|_{L^2} \le \|W^pf\|_{H^{l-p}}$, which we will now prove. First we note (see \cite[Section 7]{Schick_notes}) that on the image of $W^p$ the Sobolev and $L^2$-norms are equivalent, so it suffices to show that $c\|f\|_{L^2} \le \|W^pf\|_{L^2}$. To do so, for a $p$-simplex $\sigma$ let $U_\sigma$ be the maximal open subset of $M$ on which $\sum_{c \in \sigma} e_c = 1$ and no $e_c$ vanishes. This is nonempty, and we have $U_\sigma \cap U_\tau = \emptyset$ if $\tau \not= \sigma$ is another $p$-simplex. In addition, if $\sigma = [c_0, \ldots, c_p]$, replacing every instance of $e_{c_0}$ in $W^pf_\sigma$ with $1 - \sum_{i=1}^p e_{c_i}$ (which is valid on $U_\sigma$ by definition) we get that
\[
W^pf_\sigma = de_{c_1} \wedge \cdots \wedge de_{c_p} \text{ on } U_\sigma, 
\]
in particular it does not vanish there and so the integral of its norm on $U_\sigma$ is strictly positive. As there are only finitely many $p$-simplexes modulo $\Gamma$ and the maps $e_{\gamma c}$ are $\Gamma$-equivariant we get that there exists $a > 0$ such that
\[
\| W^p(f_\sigma \otimes v) \|_{L^2(U_\sigma)} \ge a \inf_{x \in U_\sigma} \|v\|_x. 
\]
By relative compactness of $U_\sigma$ we have that $\inf_{x \in U_\sigma} \|v\|_x > b \|\rho(\gamma)v\|$ where $\|\cdot\|$ is the norm on $\CC^2$ used to define the $L^2$-norm on $C^*(\wdt M, \rho)$, and it follows that 
\[
\| W^p(f_\sigma \otimes v) \|_{L^2(U_\sigma)} \ge a \|f_\sigma \otimes v\|_{L^2}. 
\]
Now if $f$ is an arbitrary relative cochain we can write it as
\[
f = \sum_\sigma  b_\sigma f_\sigma \otimes v_\sigma
\]
so that we have
\[
\| f \|_{L^2}^2 = \sum_\sigma b_\sigma^2 \|f_\sigma \otimes v_\sigma\|_{L^2}^2
\]
As the $U_\sigma$ are disjoint we get that 
\begin{align*}
  \| W^p(f) \|_{L^2} &\ge \sum_\sigma \| W^p(f) \|_{L^2(U_\sigma)}^2 \\
  &= \sum_\sigma \| W^p(f_\sigma \otimes v) \|_{L^2(U_\sigma)}^2 \\
  &\ge a^2 \sum_\sigma b_\sigma^2\|f_\sigma \otimes v\|_{L^2} = a^2\|f\|_{L^2}^2
\end{align*}
where the inequality on the second line follows from the fact that $W^p(f_\tau \otimes v)$ vanishes identically on $U_\sigma$, and that on the third from the previous inequality. The last line is the inequality we were after. 


%Let $\sigma$ be a simplex with vertices $c_0, \ldots, c_p$ ordered so that $c_0, \ldots, c_q$ do not lie on the boundary and the remaining do. Every form $\omega_{\sigma, c_i}$ is supported in a neighbourhood of $\sigma$ which does not intersect other $p$-simplices, so $\int_\tau W^pf_\sigma = 0$ if $\tau\not= \sigma$ (up to orientation). Now we compute $\int_\sigma W^pf_\sigma$: for convenience let $de_{\hat i}$ denote the $p$-form $\bigwedge_{j \not=i}de_{c_j}$. Then as $\sum_{i=0}^p e_{c_i} = 1$ on $\sigma$ we have for $i>0$ that
%\[de_{\hat i} = d\left(1 - \sum_{j=1}^p e_{c_j}\right) \wedge \bigwedge_{j>0, j \not= i} de_{c_j} = (-1)^i \bigwedge_{i=1}^p de_{c_i} = (-1)^i de_{\hat 0}.\]
%It follows that
%\[\int_\sigma W^pf_\sigma = p!\int_\sigma \left(\sum_{i=0}^q e_{c_i}\right) de_{\hat 0}\]
%which is equal to $1$ if $p=q$ (that is $\sigma \cap \partial\wdt M = \emptyset$). In general we denote it by $a_\sigma$ and as $\sum_{i=0}^q e_{c_i} \ge 0$ and is $>0$ on a nonempty subset of $\sigma$ we get that $a_\sigma >0$. In the basis for $C_{(2)}^p(\wdt M, \partial\wdt M)$ given by a choice of lifts of $p$-simplices from $M$ to $\wdt M$ we thus get that
%\[A^pW^p = \begin{pmatrix} a_{\sigma_1} & 0 & 0 \\ 0 & \ddots & 0 \\ 0 & 0 & a_{\sigma_{n_p}} \end{pmatrix} =: B^p.\]
%and as $a_\sigma >0$ we have $B \in \GL_{\neu\pi}(C^p(\wdt M, \partial\wdt M))$. Let $D_p$ be the differential of $H^{l-*}\Omega^*(\wdt M)$.

%The same computation as in the untwisted case shows that $A^pW^p$ is the identity map. Then $d_p = A^{p+1} \circ d_p \circ W^p$ and we can apply \cite[Lemma 2.11(9)]{Lueck} to get that the Novikov--Shubin invariants $\alpha(D_p|_{\mathrm{Im}(W)})$ and $\alpha(d_p)$ are equal. As the latter is at least $\alpha(D_p)$ and the latter is $\infty^+$ by strong acyclicity of $\rho_0$ we get that $\alpha(d_p) = \infty^+$ for all $p$, which means that all $\Delta_p$ have a spectral gap by \cite[Lemma 2.11(11)]{Lueck}. 


\subsubsection{Conclusion}

By Lemma \ref{variation_diff} the matrices $\Delta_p(\rho) \in M(n_p, \CC\pi)$ have coefficients which vary continuously for $[\rho]$ in their domain of definition $D$. In particular each map $\Delta_p \colon D \to~\mathcal B(L^2(\pi)^{n_p})$ is continuous for the operator norm topology on $\mathcal B(L^2(\pi)^{n_p})$. This is also the case for the differentials, codifferentials and Laplacians on the boundary and hence also in the relative complex $C^*(\wdt M, \partial\wdt M, \rho)$. The lemma then follows from Lemma \ref{spec_continuity} since it holds at $[\rho_0]$ by \ref{preceding}. 


%  We prove this first for $n = 1$. Let $A : \interval f01f \to \mathcal S_{\neu\pi}^{>0}(V)$ is a real-analytic path of operators. There exists an open set $\interval o01o \subset D \subset \CC$ such that $t \mapsto A(t)$ extends to a holomorphic function $D \to \mathcal S_{\neu\pi}^{>0}(V)$: by definition of a real analytic function its power series extension converges in $\mathcal B_{\neu\pi}(V)$ for $z$ in an open neighbourhood $\interval o01o \subset D_0 \subset \CC$; since $\mathcal S_{\neu\pi}^{>0}(V)$ is open we can further reduce $D_0$ to have it taking values in $\mathcal S_{\neu\pi}^{>0}(V)$. Now basic functional calculus (see eg. \cite[Theorem 6.29]{Abramovich_Aliprantis}) gives that the function 
%  \[
%  D \to \mathcal B_{\neu\pi}(V), \, z \mapsto \log A(z)
%  \]
%  is well-defined and holomorphic, and we conclude that the function $$t \mapsto \det{}_{\neu\pi} A(t) = \exp (\tr_{\neu\pi} \log A(t))$$ is real-analytic, as the restriction to the interval $\interval o01o$ of a holomorphic function.
%
%  In general this proves that the function $x \mapsto \det_{\neu\pi} A(x)$ is real-analytic on every real-analytic path contained in $U$. Now we show it is smooth on $U$. To do so we assume that there are $0 < \delta < K$ such that $\sigma(A(x)) \subset [\delta, K]$ for all $x \in U$, which is not a restriction since to prove smoothness at a point we can restrict to arbitarily small neighbourhoods. 
%  
%  Now it suffices to prove that for any function $f : \RR \to \RR$ which is smooth on $[\delta, K]$ the function $x \mapsto \tr_{\neu\pi}(f(A(x))$ is smooth (then we apply this to $\log$ for $\delta >0$). This is true by an elementary argument if $f$ is a polynomial, and we deduce the general case by approximation: if $f_n$ is a sequence of polynomials which converge $C^k$-uniformly to $f$ on $[\delta, K]$ then $f_n(A)$ converges uniformly (in the operator norm topology) to $f(A)$ on $U$ and so do its derivatives up to order $k$. The function $x \mapsto \tr_{\neu\pi}(f(A(x))$ is a uniform limit on $U$ of functions whose differentials up to order $k$ are uniformly convergent on $U$, and so is itself differentiable up to order $k$ on $U$. 
%
%  An exercise in real analysis shows that a function on $U$ which is real-analytic on every line trough a point $x$, and smooth at this point must be real-analytic on a neighbourhood of $x$\footnote{Let $f$ be such. The Taylor series of $f$ at $x$ has a positive convergence radius as it does so on every line through $x$, and by analyticity the function it defines is equal to $f$ on every line through $x$, and so they are equal up to the radius of convergence.}, and this concludes the proof. \commentleo{About the footnote: the convergence radius on any line is not uniform, so I don't understand the proof.}





